(Nearly) Optimal Private Linear Regression via Adaptive Clipping

We study the problem of differentially private linear regression where each data point is sampled from a fixed sub-Gaussian style distribution. We propose and analyze a one-pass mini-batch stochastic gradient descent method (DP-AMBSSGD) where points in each iteration are sampled without replacement. Noise is added for DP but the noise standard deviation is estimated online. Compared to existing $(\epsilon, \delta)$-DP techniques which have sub-optimal error bounds, DP-AMBSSGD is able to provide nearly optimal error bounds in terms of key parameters like dimensionality $d$, number of points $N$, and the standard deviation $\sigma$ of the noise in observations. For example, when the $d$-dimensional covariates are sampled i.i.d. from the normal distribution, then the excess error of DP-AMBSSGD due to privacy is $\frac{\sigma^2 d}{N}(1+\frac{d}{\epsilon^2 N})$, i.e., the error is meaningful when number of samples $N= \Omega(d \log d)$ which is the standard operative regime for linear regression. In contrast, error bounds for existing efficient methods in this setting are: $\mathcal{O}\big(\frac{d^3}{\epsilon^2 N^2}\big)$, even for $\sigma=0$. That is, for constant $\epsilon$, the existing techniques require $N=\Omega(d\sqrt{d})$ to provide a non-trivial result.

==> macros.tex <==
% -- algorithmic --
% \renewcommand{\algorithmicrequire}{\quad\enspace\;\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\quad\enspace\;\textbf{Effects:}}
% \renewcommand{\epsilon}{\varepsilon}
% \newcommand{\mypar}[1]{\smallskip
% 	\noindent{\textbf{{#1}:}}}
	
% \newcommand{\SUB}[1]{\hspace{-0.15in} \textbf{#1}}
% \newcommand{\mycaptionof}[2]{\captionof{#1}{#2}}

% -- author notes --
\newcommand{\anote}[1]{\todo[color=blue!30]{\tiny AT: #1}}
\newcommand{\anoteinline}[1]{\todo[color=blue!30,inline]{AT: #1}}
\newcommand{\mnote}[1]{\todo[color=green!30]{\tiny\sf BM: #1}}
\newcommand{\mnoteinline}[1]{\todo[color=green!30,inline]{BM: #1}}
\newcommand{\znote}[1]{\todo[color=green!30]{ZX: #1}}
\newcommand{\znoteinline}[1]{\todo[color=green!30,inline]{ZX: #1}}
\newcommand{\snote}[1]{\todo[color=yellow!45]{SS: #1}}
\newcommand{\snoteinline}[1]{\todo[color=yellow!45,inline]{\tiny SS: #1}}
\newcommand{\onote}[1]{\todo[color=lime!30]{OT: #1}}
\newcommand{\onoteinline}[1]{\todo[color=lime!30,inline]{\tiny OT: #1}}

\newcommand{\bnote}[1]{\todo[color=orange!30]{BB: #1}}
\newcommand{\bnoteinline}[1]{\todo[color=orange!30,inline]{\small BB: #1}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\hypersetup{final}


\newcommand{\shuffle}[1]{{\sf Shuffle}\left(#1\right)}
\newcommand{\zo}{\ensuremath{\{0,1\}}}
\newcommand{\epsl}{\epsilon_\ell}
\newcommand{\epsle}{\epsilon_{\ell e}}
\newcommand{\epslt}[1]{\epsilon_{\ell^{#1}}}
\newcommand{\epslg}[1]{\epsilon^{(\#1)}_\ell}
\newcommand{\epslgi}[1]{\epsilon^{\#1}_\ell-\infty}
\newcommand{\hepslg}[1]{\widehat{\epsilon^{\#1}_\ell}}
\newcommand{\hepslgi}[1]{\widehat{\epsilon^{\#1}_\ell-\infty}}
\newcommand{\epsc}{\epsilon_c}
\newcommand{\deltac}{\delta_c}
\newcommand{\epsr}{\epsilon_{\sf Renyi}}
% -- symbol macros --
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\newcommand{\attrfrag}{{\sf attr-frag}}
\newcommand{\recdfrag}{{\sf rept-frag}}
\newcommand{\afrag}{\ensuremath{\mathsf{att}\textsf{-}\mathsf{frag}}}
\newcommand{\rfrag}{\ensuremath{\mathsf{r}\textsf{-}\mathsf{frag}}}
\renewcommand{\vec}[1]{#1}
\newcommand{\fr}{{\texttt{fr}}\,}
\newcommand{\ir}{{\texttt{it}}\,}

% -- math macros --
\newcommand{\bolda}{\ensuremath{\boldsymbol{a}}}
\newcommand{\boldb}{\ensuremath{\boldsymbol{b}}}
\newcommand{\boldc}{\ensuremath{\boldsymbol{c}}}
\newcommand{\boldd}{\ensuremath{\boldsymbol{d}}}
\newcommand{\bolde}{\ensuremath{\boldsymbol{e}}}
\newcommand{\boldf}{\ensuremath{\boldsymbol{f}}}
\newcommand{\boldg}{\ensuremath{\boldsymbol{g}}}
\newcommand{\boldh}{\ensuremath{\boldsymbol{h}}}
\newcommand{\boldi}{\ensuremath{\boldsymbol{i}}}
\newcommand{\boldj}{\ensuremath{\boldsymbol{j}}}
\newcommand{\boldk}{\ensuremath{\boldsymbol{k}}}
\newcommand{\boldl}{\ensuremath{\boldsymbol{l}}}
\newcommand{\boldm}{\ensuremath{\boldsymbol{m}}}
\newcommand{\boldn}{\ensuremath{\boldsymbol{n}}}
\newcommand{\boldo}{\ensuremath{\boldsymbol{o}}}
\newcommand{\boldp}{\ensuremath{\boldsymbol{p}}}
\newcommand{\boldq}{\ensuremath{\boldsymbol{q}}}
\newcommand{\boldr}{\ensuremath{\boldsymbol{r}}}
\newcommand{\bolds}{\ensuremath{\boldsymbol{s}}}
\newcommand{\boldt}{\ensuremath{\boldsymbol{t}}}
\newcommand{\boldu}{\ensuremath{\boldsymbol{u}}}
\newcommand{\boldv}{\ensuremath{\boldsymbol{v}}}
\newcommand{\boldw}{\ensuremath{\boldsymbol{w}}}
\newcommand{\boldx}{\bfx}
\newcommand{\boldy}{\ensuremath{\boldsymbol{y}}}
\newcommand{\boldz}{\ensuremath{\boldsymbol{z}}}
\newcommand{\boldzero}{\ensuremath{\boldsymbol{0}}}
\newcommand{\boldone}{\ensuremath{\boldsymbol{1}}}

\newcommand{\boldA}{\ensuremath{\boldsymbol{A}}}
\newcommand{\boldB}{\ensuremath{\boldsymbol{B}}}
\newcommand{\boldC}{\ensuremath{\boldsymbol{C}}}
\newcommand{\boldD}{\ensuremath{\boldsymbol{D}}}
\newcommand{\boldE}{\ensuremath{\boldsymbol{E}}}
\newcommand{\boldF}{\ensuremath{\boldsymbol{F}}}
\newcommand{\boldG}{\ensuremath{\boldsymbol{G}}}
\newcommand{\boldH}{\ensuremath{\boldsymbol{H}}}
\newcommand{\boldI}{\ensuremath{\boldsymbol{I}}}
\newcommand{\boldJ}{\ensuremath{\boldsymbol{J}}}
\newcommand{\boldK}{\ensuremath{\boldsymbol{K}}}
\newcommand{\boldL}{\ensuremath{\boldsymbol{L}}}
\newcommand{\boldM}{\ensuremath{\boldsymbol{M}}}
\newcommand{\boldN}{\ensuremath{\boldsymbol{N}}}
\newcommand{\boldO}{\ensuremath{\boldsymbol{O}}}
\newcommand{\boldP}{\ensuremath{\boldsymbol{P}}}
\newcommand{\boldQ}{\ensuremath{\boldsymbol{Q}}}
\newcommand{\boldR}{\bfR}
\newcommand{\boldS}{\ensuremath{\boldsymbol{S}}}
\newcommand{\boldT}{\ensuremath{\boldsymbol{T}}}
\newcommand{\boldU}{\ensuremath{\boldsymbol{U}}}
\newcommand{\boldV}{\ensuremath{\boldsymbol{V}}}
\newcommand{\boldW}{\ensuremath{\boldsymbol{W}}}
\newcommand{\boldX}{\ensuremath{\boldsymbol{X}}}
\newcommand{\boldY}{\ensuremath{\boldsymbol{Y}}}
\newcommand{\boldZ}{\ensuremath{\boldsymbol{Z}}}

\newcommand{\bfA}{\ensuremath{\mathbf{A}}}
\newcommand{\bfB}{\ensuremath{\mathbf{B}}}
\newcommand{\bfC}{\ensuremath{\mathbf{C}}}
\newcommand{\bfD}{\ensuremath{\mathbf{D}}}
\newcommand{\bfE}{\ensuremath{\mathbf{E}}}
\newcommand{\bfF}{\ensuremath{\mathbf{F}}}
\newcommand{\bfG}{\ensuremath{\mathbf{G}}}
\newcommand{\bfH}{\ensuremath{\mathbf{H}}}
\newcommand{\bfI}{\ensuremath{\mathbf{I}}}
\newcommand{\bfJ}{\ensuremath{\mathbf{J}}}
\newcommand{\bfK}{\ensuremath{\mathbf{K}}}
\newcommand{\bfL}{\ensuremath{\mathbf{L}}}
\newcommand{\bfM}{\ensuremath{\mathbf{M}}}
\newcommand{\bfN}{\ensuremath{\mathbf{N}}}
\newcommand{\bfO}{\ensuremath{\mathbf{O}}}
\newcommand{\bfP}{\ensuremath{\mathbf{P}}}
\newcommand{\bfQ}{\ensuremath{\mathbf{Q}}}
\newcommand{\bfR}{\ensuremath{\mathbf{R}}}
\newcommand{\bfS}{\ensuremath{\mathbf{S}}}
\newcommand{\bfT}{\ensuremath{\mathbf{T}}}
\newcommand{\bfU}{\ensuremath{\mathbf{U}}}
\newcommand{\bfV}{\ensuremath{\mathbf{V}}}
\newcommand{\bfW}{\ensuremath{\mathbf{W}}}
\newcommand{\bfX}{\ensuremath{\mathbf{X}}}
\newcommand{\bfY}{\ensuremath{\mathbf{Y}}}
\newcommand{\bfZ}{\ensuremath{\mathbf{Z}}}

\newcommand{\bfa}{\ensuremath{\mathbf{a}}}
\newcommand{\bfb}{\ensuremath{\mathbf{b}}}
\newcommand{\bfc}{\ensuremath{\mathbf{c}}}
\newcommand{\bfd}{\ensuremath{\mathbf{d}}}
\newcommand{\bfe}{\ensuremath{\mathbf{e}}}
\newcommand{\bff}{\ensuremath{\mathbf{f}}}
\newcommand{\bfg}{\ensuremath{\mathbf{g}}}
\newcommand{\bfh}{\ensuremath{\mathbf{h}}}
\newcommand{\bfi}{\ensuremath{\mathbf{i}}}
\newcommand{\bfj}{\ensuremath{\mathbf{j}}}
\newcommand{\bfk}{\ensuremath{\mathbf{k}}}
\newcommand{\bfl}{\ensuremath{\mathbf{l}}}
\newcommand{\bfm}{\ensuremath{\mathbf{m}}}
\newcommand{\bfn}{\ensuremath{\mathbf{n}}}
\newcommand{\bfo}{\ensuremath{\mathbf{o}}}
\newcommand{\bfp}{\ensuremath{\mathbf{p}}}
\newcommand{\bfq}{\ensuremath{\mathbf{q}}}
\newcommand{\bfr}{\ensuremath{\mathbf{r}}}
\newcommand{\bfs}{\ensuremath{\mathbf{s}}}
\newcommand{\bft}{\ensuremath{\mathbf{t}}}
\newcommand{\bfu}{\ensuremath{\mathbf{u}}}
\newcommand{\bfv}{\ensuremath{\mathbf{v}}}
\newcommand{\bfw}{\ensuremath{\mathbf{w}}}
\newcommand{\bfx}{\ensuremath{\mathbf{x}}}
\newcommand{\bfy}{\ensuremath{\mathbf{y}}}
\newcommand{\bfz}{\ensuremath{\mathbf{z}}}

\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calJ}{\ensuremath{\mathcal{J}}}
\newcommand{\calK}{\ensuremath{\mathcal{K}}}
\newcommand{\calL}{\ensuremath{\mathcal{L}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calO}{\ensuremath{\mathcal{O}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
\newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calW}{\ensuremath{\mathcal{W}}}
\newcommand{\calX}{\ensuremath{\mathcal{X}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\calZ}{\ensuremath{\mathcal{Z}}}

% -- text in math mode --
\newcommand{\textpoly}[0]{{\rm poly}}
\newcommand{\poly}[1]{\ensuremath{{\rm poly}\left(#1\right)}}
\newcommand{\polylog}[1]{\ensuremath{{\rm polylog}\left(#1\right)}}
\renewcommand{\Pr}{\mathop{\mathbf{Pr}}}
\renewcommand{\th}{\ensuremath{^{\rm th}}} % ordinal numbers
\newcommand{\mystar}[1]{\ensuremath{#1^*}}
\newcommand{\E}{\mathop{\mathbf{E}}}
\newcommand{\BiasedSampling}{\mathsf{BiasedSampling}}
\newcommand{\R}{\mathbb{R}}


% --theorem --
\newtheorem{lem}{Lemma}[section]
\newtheorem{strlem}[lem]{Structural Lemma}
\newtheorem{thm}[lem]{Theorem}
\newtheorem{cor}[lem]{Corollary}
\newtheorem{problem}[lem]{Problem}
\newtheorem{defn}[lem]{Definition}
\newtheorem{fact}[lem]{Fact}
\newtheorem{prop}[lem]{Proposition}
%\newtheorem{example}{Example}
\newtheorem{assumption}[lem]{Assumption}
\newtheorem{claim}[lem]{Claim}
\newtheorem{definition}[lem]{Definition}

% -- for record fragmentation (from shuangsong) --
\newcommand{\rr}{\text{rr}}
\newcommand{\rrt}{\text{rr3}}
\newcommand{\rrzo}{\text{rr01}}
\newcommand{\mse}{\text{MSE}}
\newcommand{\rmse}{\textsc{RMSE}}
\newcommand{\nrmse}{\text{noise}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\bracket}[1]{\left(#1\right)}
\newcommand{\sqbracket}[1]{\left[#1\right]}
\newcommand{\nbr}[1]{\num[group-separator={,}]{#1}}
\makeatletter
\newcommand{\vast}{\bBigg@{4}}
\newcommand{\Vast}{\bBigg@{5}}
\makeatother

\newcommand{\crowd}{\sf cr}

\newcommand{\Var}[1]{\ensuremath{\mathbf{Var}\left(#1\right)}}
\newcommand{\Cov}[2]{\ensuremath{\mathbf{Cov}\left(#1, #2\right)}}
\newcommand{\Mean}[1]{\ensuremath{\mathbf{Mean}\left(#1\right)}}
\newcommand{\expt}[2]{\E_{#1}\left[{#2}\right]}
\newcommand{\power}[2]{\left(#1\right)^{#2}}
\newcommand{\indi}[1]{\mathbbm{1}\left(#1\right)}
\newcommand{\ip}[2]{\left\langle #1, #2\right\rangle}
\newcommand{\ipn}[3]{\langle #1, #2\rangle_{#3}}
\newcommand{\voc}[0]{\calD}
\newcommand{\vocs}[0]{k}
\newcommand{\hpick}[0]{\hat{\ell}}
\newcommand{\htotal}[0]{\ell}
\newcommand{\sks}[0]{\kappa}
\newcommand{\calLH}{\calL_\texttt{Huber}\,}
\newcommand{\privT}{\Theta^\texttt{priv}\,}
\newcommand{\privV}{\bfV^\texttt{priv}\,}
\newcommand{\thetaH}{\theta^\texttt{Huber}\,}
\newcommand{\ltwo}[1]{\left\|#1\right\|_2}
\newcommand{\snorm}[2]{\left\|#1\right\|_{#2}}
\newcommand{\blah}{{\color{red} BLAH}\,}
\newcommand{\norm}[1]{\| #1 \|}

\newcommand{\trunc}[2]{\left[#2\right]_{#1}}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\newcommand{\bbracket}[1]{\left\{#1\right\} }
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2%
}
\newcommand{\infdiv}{D\infdivx}
\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}


% -- references and labels (eq. fig., ...) --


\newcommand{\sref}[1]{{Sec}~\ref{#1}}
\newcommand{\fref}[1]{{Fig}~\ref{#1}}
\newcommand{\eref}[1]{{Eq}~\ref{#1}}
\newcommand{\tref}[1]{{Table}~\ref{#1}}
\newcommand{\aref}[1]{{Algorithm}~\ref{#1}}

\newcommand{\regret}[2]{{\sf Regret}_T(#1;#2)\,}

\newcommand{\mypar}[1]{\smallskip
	\noindent{\textbf{{#1}:}}}
	
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\nadagrad}{\calA_{\sf noisy-AdaGrad}\,}

\newcommand{\apriv}{\calA_{\sf priv}\,}
\newcommand{\risk}[1]{{\sf Risk}(#1)\,}
\newcommand{\ptheta}{\theta_{\sf priv}\,}
\renewcommand{\tilde}{\widetilde}
\newcommand{\aftrl}{\calA_{\sf FTRL}}
\newcommand{\aftrlprox}{\calA_{\sf FTRL}^{\sf Prox}\,}
\newcommand{\poprisk}[1]{{\sf PopRisk}(#1)\,}
\newcommand{\tree}{\calT}
\newcommand{\init}{{\texttt{InitializeTree}}\,}
\newcommand{\addt}{{\texttt{AddToTree}}\,}
\newcommand{\gett}{{\texttt{GetSum}}\,}
\newcommand{\outputt}{{\bf Output}\,}
\newcommand{\node}{\texttt{node}}
\newcommand{\thetanp}{\theta^{\sf np}}
\newcommand{\npJ}{J_t^{\sf np}}
\newcommand{\linL}{\calL^{\sf lin}}
\newcommand{\pJ}{J_t^{\sf priv}}
\newcommand{\Ex}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\thetash}{\widetilde{\theta}}
\newcommand{\opt}{{\sf OPT\,}}
\newcommand{\dm}{p}
\newcommand{\U}[1]{\bfU_{#1}}
\newcommand{\baseU}{\bfU_{\sf base}}
\newcommand{\calLpop}{\calL_{\sf pop}}
\newcommand{\riskP}{{\sf Risk_{\texttt{Pop}}}}
\newcommand{\bill}{\calB}
\newcommand{\adptasgd}{\calA_{\sf DP-TASGD}}

\newcommand{\dpnoise}{{\alpha}}
\newcommand{\tOmega}{\widetilde{\Omega}}
